X-Eval: Generalizable Multi-aspect Text Evaluation via Augmented Instruction Tuning with Auxiliary Evaluation Aspects

Natural Language Generation (NLG) typically involves evaluating the generated text in various aspects (e.g., consistency and naturalness) to obtain a comprehensive assessment. However, multi-aspect evaluation remains challenging as it may require the evaluator to generalize to any given evaluation aspect even if it's absent during training. In this paper, we introduce X-Eval, a two-stage instruction tuning framework to evaluate the text in both seen and unseen aspects customized by end users. X-Eval consists of two learning stages: the vanilla instruction tuning stage that improves the model's ability to follow evaluation instructions, and an enhanced instruction tuning stage that exploits the connections between fine-grained evaluation aspects to better assess text quality. To support the training of X-Eval, we collect AspectInstruct, the first instruction tuning dataset tailored for multi-aspect NLG evaluation spanning 27 diverse evaluation aspects with 65 tasks. To enhance task diversity, we devise an augmentation strategy that converts human rating annotations into diverse forms of NLG evaluation tasks, including scoring, comparison, ranking, and Boolean question answering. Extensive experiments across three essential categories of NLG tasks: dialogue generation, summarization, and data-to-text coupled with 21 aspects in meta-evaluation, demonstrate that our X-Eval enables even a lightweight language model to achieve a comparable if not higher correlation with human judgments compared to the state-of-the-art NLG evaluators, such as GPT-4.

==> backup.tex <==

% ------ backup for section 6.1

% Notably, \method{} consistently outperforms the baseline metrics in the top section, achieving an average improvement exceeding 45\% in Spearman correlation. This highlights \method{}'s superior adaptability to unseen aspects in comparison to traditional metrics and evaluators of similar model size. Moreover, \method{}, with a modest 780M parameter size, shows performance on par with the proprietary LLM-based baselines shown in the middle section of the table. 
% The bottom section of the table provides a comparison among different variants of \method{}. ``\method{} w/o Training'' exhibits a sub-optimal average correlation, even when inference with identical instructions, highlighting the importance of finetuning on \evalinstruct{}. 
% By comparing the correlations between \method{} and ``\method{} w/o Instructions'', we observe a clear performance drop after removing detailed evaluation instructions during training, indicating the effectiveness of instruction tuning on comprehensive evaluation instructions.
% \lifu{FlanT5 is also an instruction tuned model. Why does it perform such worse than our approach? what are the main problems? Need to provide more in-depth analysis.}
% Furthermore, the average correlation of \method{} improves from $0.342$ to $0.383$ with the inclusion of the second training stage, emphasizing the effectiveness of the auxiliary aspects in evaluation.
